Neural Temporal Point Processes For Modelling Electronic Health Records

The modelling of Electronic Health Records (EHRs) has the potential to drive more efficient allocation of healthcare resources, enabling early intervention strategies and advancing personalised healthcare. However, EHRs are challenging to model due to their realisation as noisy, multi-modal data occurring at irregular time intervals. To address their temporal nature, we treat EHRs as samples generated by a Temporal Point Process (TPP), enabling us to model what happened in an event with when it happened in a principled way. We gather and propose neural network parameterisations of TPPs, collectively referred to as Neural TPPs. We perform evaluations on synthetic EHRs as well as on a set of established benchmarks. We show that TPPs significantly outperform their non-TPP counterparts on EHRs. We also show that an assumption of many Neural TPPs, that the class distribution is conditionally independent of time, reduces performance on EHRs. Finally, our proposed attention-based Neural TPP performs favourably compared to existing models, whilst aligning with real world interpretability requirements, an important step towards a component of clinical decision support systems.

==> preamble/acronyms/f.tex <==
\newacronym{fs}{FS}{FastSent}
\newacronym{ft}{FT}{Fourier Transform}

==> preamble/style.tex <==
% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2020

% ready for submission
 % \usepackage{neurips_2020}

% to compile a preprint version, e.g., for submission to arXiv, add add the
% [preprint] option:
%     \usepackage[preprint]{neurips_2020}

% to compile a camera-ready version, add the [final] option, e.g.:
% \usepackage[preprint]{neurips_2020}

%     to avoid loading the natbib package, add option nonatbib:
% \usepackage{neurips_2020}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{subcaption}
\usepackage{bbm}
\usepackage[pdftex,
            pdfauthor={Anonymous},
            pdftitle={Neural Temporal Point Processes for Modelling Electronic Health Records}]{hyperref}


==> sections/authors.tex <==
% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to break the
% lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% authors names on the first line, and the last on the second line, try using
% \AND instead of \And before the third author name.

\author{%
  Joseph Enguehard\thanks{Equal contribution.
  Joseph Enguehard and Dan Busbridge led the research, implemented the models and performed the experiments.
  Adam Bozson created the synthetic EHR datasets and provided insights during project inception.
  Claire Woodcock strategically guided the project and contributed the broader impact statement.
  Nils Y. Hammerla provided technical guidance throughout.} \,\thanks{Corresponding author, address:
  \href{mailto:joseph.enguehard@babylonhealth.com}{\texttt{joseph.enguehard@babylonhealth.com}}.} \\
  Babylon Health\\
  \And
  Dan Busbridge$^*$\thanks{Now at Apple.}\\
  Babylon Health\\
  \And
  Adam Bozson \\
  Babylon Health\\
  \And
  Claire Woodcock \\
  Babylon Health\\
  \And
  Nils Y. Hammerla \\
  Babylon Health
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
  % \AND
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
  % \And
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
  % \And
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
}

